Characterizing Truthful Multi-Armed Bandit Mechanisms

We consider a multi-round auction setting motivated by pay-per-click auctions for Internet advertising. In each round the auctioneer selects an advertiser and shows her ad, which is then either clicked or not. An advertiser derives value from clicks; the value of a click is her private information. Initially, neither the auctioneer nor the advertisers have any information about the likelihood of clicks on the advertisements. The auctioneer's goal is to design a (dominant strategies) truthful mechanism that (approximately) maximizes the social welfare. If the advertisers bid their true private values, our problem is equivalent to the "multi-armed bandit problem", and thus can be viewed as a strategic version of the latter. In particular, for both problems the quality of an algorithm can be characterized by "regret", the difference in social welfare between the algorithm and the benchmark which always selects the same "best" advertisement. We investigate how the design of multi-armed bandit algorithms is affected by the restriction that the resulting mechanism must be truthful. We find that truthful mechanisms have certain strong structural properties -- essentially, they must separate exploration from exploitation -- and they incur much higher regret than the optimal multi-armed bandit algorithms. Moreover, we provide a truthful mechanism which (essentially) matches our lower bound on regret.

==> app-PSim.tex <==
\section{Algorithm \PSim{} is strongly separated}
\label{app:PSim}


We consider \PSim~\cite{Bobby-stoc04-journal-version,Robert-Kleinberg-Lecture-8}, an algorithm for the adversarial MAB problem which we interpret here as an MAB allocation rule. We show that \PSim{} is strongly separated, which implies
Corollary~\ref{cor:weakly-truthful}.

For the sake of completeness, let us present \PSim{}. As usual, $k$ denotes the number of agents; let $[k]$ denote the set of agents.

\smallskip
\begin{compactenum}
\item[\bf Input:] Time horizon $T$, bid vector $b$. Let $\vmax=\max_{i}b_{i}$.
\item[\bf Output:] For each round $t\leq T$, a distribution on $[k]$.
\item Divide the time horizon into $P$ phases of $T/P$ consecutive rounds each.
\begin{comment}
%\item Pick number of phases $P$ and $Q=T/P$. Divide the time horizon into $P$ phase of length $Q$ each. For phase $p=1,2,\dots,P$, let $\phi_p$ denote the sequence of rounds in phase $p$. That is
	$$\phi_p=\{(p-1)Q+1,\; (p-1)Q+2  \LDOTS\ pQ\}.$$
\end{comment}
%\item For each phase $\phi_p$, pick a random one-to-one function $f_p:K\to \phi_p$, and call $f_p(K)$ as exploration rounds in phase $p$.
\item From rounds of each phase $p$, pick without replacement $k$ rounds at random (called the {\em exploration rounds}) and assign them randomly to $k$ arms. Let $S$ denote the set of all exploration rounds (of all phases). Let $f:S\to [k]$ be the function which tells which arm is assigned to an exploration round in $S$. The rounds in $[T]\setminus S$ are called the exploitation rounds.
%and rounds $S_i:=\cup_{p}f_p(i)$ as exploration rounds for agent $i$.
\item Let $w_i(0)=1$ for all $i\in [k]$.
\item For each phase $p=1,2,\dots,P$
	\begin{compactenum}
	\item For each round $t$ in phase $p$	
		\begin{compactenum}
		\item If $t\in S$ and $f(t)=i$, then define the distribution $\gamma(b;t;S,f)$ such that $\gamma_i(b;t;S,f)=1$. Pick an agent according to this distribution (equivalently, pick agent $i$), observe the click $\rho_i(t)$, and update $w_i(p)$ multiplicatively,
    $$w_i(p)=w_i(p-1)\cdot (1+\epsilon)^{\rho_i(t) b_i/\vmax}.$$
		\item If $t\not\in S$, then define the distribution $\gamma(b;t;S,f)$ such that $\gamma_i(b;t;S,f)=\frac{w_i(p-1)}{\sum_{j}w_j(p-1)}$. Pick an agent according to $\gamma(b;t;S,f)$, observe the feedback, and discard the feedback.
		\end{compactenum}
	\end{compactenum}
\end{compactenum}
If we pick the values $\epsilon=(k\log k/T)^{1/3}$ and $P=(\log k)^{1/3}(T/k)^{2/3}$, then the regret of $\psim$ is bounded by $\bigo((k\log k)^{1/3}T^{2/3}\vmax)$ against any oblivious adversary (see \cite{Bobby-stoc04-journal-version,Robert-Kleinberg-Lecture-8}).

\begin{claim}
$\psim$ is strongly-separated.
\end{claim}

\begin{proof}
It is clear from the structure of $\psim$ above that it chooses a set $S$ of exploration rounds and a function $f:S\to [k]$ in the beginning without looking at the bids and then runs an $(S,f)$-separated allocation. We need to prove that the $(S,f)$-separated allocation is pointwise monotone. For this we need prove that the probability $\gamma_i(b;t; S,f)$ is monotone in the bid of agent $i$, where $\gamma_i(b;t;S,f)$ denotes the probability of picking agent $i$ in round $t$ when bids are $b$ given the choice of $S$ and $f$. If $t\in S$, the $\gamma_i(b;t;S,f)$ is independent of bids, and hence is monotone in $b_i$. Let $t\not\in S$ and $t$ is a round in phase $p$. Let us denote by $f^{-1}(i,p)$ the (unique) exploration round in phase $p$ assigned to agent $i$. We then have
\begin{align*}
\gamma_i(b;t; S,f) = (1+\epsilon)^{\frac{b_i}{\vmax}\sum_{q=1}^{p-1}\rho_i(f^{-1}(i,q))} \biggm/ \sum_{j}(1+\epsilon)^{\frac{b_j}{\vmax}\sum_{q=1}^{p-1}\rho_j(f^{-1}(j,q))}.
\end{align*}
We split the denominator into the term for agent $i$ and all other terms. It is then not hard to see that this is a non-decreasing function of $b_i$.
\end{proof}



==> app-characterization.tex <==
\section{The ``only if" direction of Theorem~\ref{thm:characterization-k-non-scalefree}}
\label{app:characterization}


\begin{lemma}
\label{lemma:truthful-implies-influential-is-secured}
Consider the \problem. Let $(\A,\mathcal{P})$ be a normalized truthful mechanism such that $\A$ is a non-degenerate deterministic allocation rule. Then \A\ is weakly separated.
\end{lemma}
\begin{proof}
Assume $\A$ is not weakly separated. Then there is a \emph{counterexample} $(\rho,b,t,t',i)$: a \realization $\rho$, bid vector $b$, rounds $t,t'$ and agent $i$ such that round $t$ is $(b;\rho)$-influential with influenced agent $i$ and influenced round $t'$  and it does not holds that round $t$ is $(b;\rho)$-secured from $i$. We prove that this leads to a contradiction..

Let us pick a counterexample $(\rho,b,t,t',i)$ with a minimum value of $t'$ over all choices of $(\rho,b,t,i)$. Without loss of generality, let us assume that $\rho_i(t')=1$ and $\rho_j(t'')=0$ for all $t''>t'$ and for all agents $j$.

Let $j = \A(b;\rho;t)$. As it does not holds that round $t$ is $(b;\rho)$-secured from $i$, this means that $j\neq i$, and
there exists a bid $b^+_i>b_i$ such that $\A(b^+_i,b_{-i};\rho;t)\neq j$.
% Thus conclude that there exists a bid $b_i^+ > b_i$ for agent $i\not=\A(b;\rho;t)$, such that $\A(b_i^+, b_{-i}; \rho; t)\neq j$.

Let $\rho'=\rho\xor\indicator(j,t)$. The mechanism needs to compute prices for agent $i$ when her bid is $b_i^+$ under \realizations $\rho$ and $\rho'$, that is to compute
    $\price_i(b_i^{+}, b_{-i}; \rho)$
and
    $\price_i(b_{i}^{+}, b_{-i}; \rho')$.
Therefore, the mechanism needs to compute the integral
     $I_i(\varphi) = \int_{x \leq b^+_1} \mathcal{C}_i(x, b_{-i};\varphi) \d x$
for both \realizations $\varphi \in \{\rho, \rho'\}$.


First of all, for all $x\leq b_i^+$ and for all $t''<t'$, $\A_i(x,b_{-i}; \rho; t'')=\A_i(x,b_{-i};\rho'; t'')$. If not,then the minimality of $t'$ will be violated. This is because, if there were such an $x$ and $t''<t'$ with $\A_i(x,b_{-i};\rho;t'')\not= \A_i(x,b_{-i};\rho';t'')$, then round $t$ will still be $(b,\rho)$-influential with influenced agent $i$, and influenced round $t''<t'$, violating the minimality of $t''$. Therefore, when we decrease the bid of agent $i$, the only difference in the allocation can occur at time round $t'$.

As $i$ is the influenced agent at round $t'$ it must hold that $\A_i(b_i,b_{-i};\rho;t')\neq \A_i(b_i,b_{-i};\rho',t')$.
Let us assume $0=\A_i(b_i,b_{-i};\rho;t') < \A_i(b_i,b_{-i};\rho',t')=1$ (otherwise, we can swap $\rho$ and $\rho'$). Note that we have made use of the fact that the mechanism is deterministic. Let us make the the claim that for all bids $x\leq b^+_i$ the influence of round $t$ on round $t'$ is in the same ``direction.''
\begin{align}\label{eq:influences-in-same-direction-k-players}
\A_i(x,b_{-i};\rho;t')\leq \A_i(x,b_{-i}; \rho'; t')
    \text{~~for all $x\leq b_i^+$}.
\end{align}
Suppose~\refeq{eq:influences-in-same-direction-k-players} does not hold. Then there is an $x\leq b_i^+$ such that $1=\A_i(x,b_{-i};\rho;t')>\A_i(x,b_{-i};\rho';t')=0$. (Note that we have used the fact that the mechanism is deterministic.) If $x>b_i$, then pointwise monotonicity is violated in $\rho'$, since $0=\A_i(x,b_{-i};\rho';t')<\A_i(b_{i},b_{-i};\rho';t')=1$. If $x<b_i$ on the other hand, then the pointwise-monotonicity is violated in $\rho$, since $1=\A_i(x,b_{-i};\rho;t')>\A_i(b_i,b_{-i};\rho;t')=0$, giving a contradiction in both cases. The claim~\refeq{eq:influences-in-same-direction-k-players} follows.

By the non-degeneracy of \A, there exists a non-degenerate interval $I$ containing $b_i$ such that
\begin{align}\label{eq:influence-positive}
\A_i(x,b_{-i};\rho;t')<\A_i(x,b_{-i};\rho';t')
\text{~~for all $x\in I$}.
\end{align}
By~\refeq{eq:influences-in-same-direction-k-players} and ~\refeq{eq:influence-positive} it follows that
    $I_i(\rho) < I_i(\rho') $.
However, the mechanism cannot distinguish between $\rho$ and $\rho'$ when agent $i$'s bid is $b_i^+$, since the differing bit $\rho_j(t)$ is not seen. Contradiction.
\end{proof}




==> app-ucb-counterexample.tex <==
\section{UCB1 is not truthful}

In this section, we informally show that a simple adaptation of well-known $\ucbone$ algorithm \cite{bandits-ucb1} is not truthful for \problem. We will first describe a natural adaptation of the $\ucbone$ algorithm to make it into a mechanism and then show that prices cannot be computed to make it truthful.

\paragraph{$\ucbone$ mechanism}
The mechanism is given the bids $b_1, b_2, \dots, b_k$. Define $n_{i,t}$ to be the number of times agent $i$ has been selected up to time $t$, and let $\mubar_{i,t}$ be the empirical click-through rate for agent $i$ up to time $t$ (this is the number of clicks agent $i$ has gotten divided by $n_{i,t}$). Also define $r_{i,t}=\sqrt{\frac{8\log t}{n_{i,t}}}$.

In each time step $t+1$, the mechanism shows the agent
\begin{align*}
i^*_{t+1} = \arg\max_{i\in K} \left( \left( \mubar_{i,t} + r_{i,t} \right) \cdot b_i \right),
\end{align*}
with the convention $0/0=0$ and $1/0=\infty$.

We note that the mechanism described above is monotone (in expectation) in $b_{i}$ for each agent $i$. That is, the expected number of clicks received by each agent is a monotone non-decreasing function of her bid.
\yoginote{I have been trying for some time to prove it, but it seems harder than I thought it would be. I am not even sure whether I should claim its monotonicity.}
Because of the monotonicity, we know from Theorem~\ref{thm:Myerson-characterization} that there exists prices that make it into a truthful mechanism, and they are computable for each realization, if we know the {\em whole} realization. In particular, for agent $i$, the price must be
\begin{align*}
p_{i}(b_{i},b_{-i};\rho) = \E[c_i(b_i)] \cdot b_i - \int_{x=0}^{b_i}\E[c_{i}(x)] \d x,
\end{align*}
where the expectation is taken over realizations.


\begin{comment}
There are two natural ways to charge the price. If the price is charge on a per round basis, then agent $i^*$ is charged $(\mubar_{i^*,t}+r_{i^*,t})b_{i^*}/\arg\max_{i\in K-\{i^*\}}(\mubar_{i,t}+r_{i,t})$ if she gets a click, and $0$ otherwise. If the price is charge once at the end of the time horizon for all clicks, then to charge price for round $t$, the CTR estimates that are available at the end of the time horizon are used, rather than those at time round $t$.
\yoginote{Does the second method of charging prices make sense?}
\end{comment}

\paragraph{$\ucbone$ is far from being truthful}
The mechanism described above is very far from being truthful. To see this, order the agents in decreasing order of $\mu_i v_i$. It is clear that once the maximum ``upper confidence bound'' of agents $2$ up to $n$ (that is $\max_{i=2,\dots,n}(\mubar_{i,t} + r_{i,t})v_i$) becomes less than $(\mu_1)\cdot v_1$, agent 1 will always be shown from that point onwards. The radius $r_{1,t}$ of agent $1$ will keep shrinking as a result, but the radius of other agents will not change. As a result, agent $1$ will pay close to $v_1$ for each click she receives (since $(\mubar_{1,t}+r_{1,t})v_{1}$ will be slightly larger than $\mu_{1}v_1$, and $\max_{i=2,\dots,n}(\mubar_{i,t}+r_{i,t})v_i$ will be slightly smaller than $\mu_{1}v_{1}$, and agent $1$ pays the ratio times $v_1$). This is essentially the first price.

Therefore, there is a big incentive for agent $1$ to underbid so as to pay less once the mechanism figures out that she is the socially-optimal agent. (Of course, if agent $1$ underbids, then it takes longer for mechanism to figure out that she is the best agent.)

